Penalty Alternating Direction Methods for Mixed-Integer Optimization: A New View on Feasibility Pumps

Feasibility pumps are highly effective primal heuristics for mixed-integer linear and nonlinear optimization. However, despite their success in practice there are only few works considering their theoretical properties. We show that feasibility pumps can be seen as alternating direction methods applied to special reformulations of the original problem, inheriting the convergence theory of these methods. Moreover, we propose a novel penalty framework that encompasses this alternating direction method, which allows us to refrain from random perturbations that are applied in standard versions of feasibility pumps in case of failure. We present a convergence theory for the new penalty based alternating direction method and compare the new variant of the feasibility pump with existing versions in an extensive numerical study for mixed-integer linear and nonlinear problems.

==> imgs/minlplib_instance_table.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-0 package
% Mon Oct 24 11:24:24 2016
\begin{longtable}{lrrrr}
\caption{Detailed numerical results for the penalty ADM based feasibility pump on all 263 \MINLPLib instances with integer variables. Objective function value, running times (s), outer penalty iterations (\#Pen.), and inner ADM iterations (\#ADM) for the method with $\lambda = 0.9$, additive penalty parameter update rule~$\inc_{\text{a}}$, and deactivated local branching.} \\ 
  \toprule
Instance & Objective & Time & \#Pen. & \#ADM \\ 
  \midrule
\endhead
\bottomrule
\endfoot
4stufen & 118114.00 & 9.00 &  74 & 169 \\ 
  alan & 3.00 & 1.00 &   5 &   7 \\ 
  batch & 309205.00 & 2.00 &  22 &  43 \\ 
  batchdes & 185769.00 & 1.00 &   7 &  13 \\ 
  beuster & 128512.00 & 17.00 &  99 & 254 \\ 
  blendgap & -0.00 & 1.00 &   1 &   1 \\ 
  cecil\_13 & -115564.00 & 8.00 &  65 &  92 \\ 
  chp\_partload & --- & --- & 25022 & 25231 \\ 
  contvar & 829318.00 & 7.00 &   8 &  35 \\ 
  csched1 & -30174.60 & 0.00 &   4 &   5 \\ 
  csched1a & -29903.30 & 0.00 &   7 &  13 \\ 
  csched2 & -160668.00 & 2.00 &   9 &  20 \\ 
  csched2a & -162047.00 & 7.00 &  44 & 120 \\ 
  deb10 & 209.43 & 1.00 &   9 &  13 \\ 
  deb6 & 251.66 & 1.00 &   3 &   4 \\ 
  deb7 & 176.08 & 2.00 &   3 &   4 \\ 
  deb8 & 176.08 & 3.00 &   3 &   4 \\ 
  deb9 & 176.08 & 2.00 &   3 &   4 \\ 
  dosemin2d & 173.98 & 11.00 &   5 &  11 \\ 
  dosemin3d & 1.32 & 30.00 &   7 &  13 \\ 
  du-opt & 5.34 & 0.00 &   3 &   4 \\ 
  du-opt5 & 112.02 & 1.00 &   5 &   8 \\ 
  eg\_all\_s & 8.67 & 13.00 &  20 &  44 \\ 
  eg\_disc2\_s & 5.68 & 3.00 &   3 &   4 \\ 
  eg\_disc\_s & 6.03 & 6.00 &   7 &  15 \\ 
  eg\_int\_s & 8.32 & 6.00 &   6 &  13 \\ 
  elf & 1.68 & 0.00 &   1 &   1 \\ 
  eniplac & -120713.00 & 42.00 & 636 & 764 \\ 
  enpro48pb & 188887.00 & 1.00 &  10 &  23 \\ 
  enpro56pb & 266762.00 & 3.00 &  24 &  56 \\ 
  ex1221 & 7.67 & 0.00 &   1 &   1 \\ 
  ex1222 & 1.08 & 1.00 &   6 &  10 \\ 
  ex1223 & 5.81 & 0.00 &   6 &  10 \\ 
  ex1223a & 5.81 & 1.00 &   5 &   8 \\ 
  ex1223b & 5.81 & 0.00 &   6 &  10 \\ 
  ex1224 & -0.88 & 1.00 &  12 &  19 \\ 
  ex1225 & 31.00 & 1.00 &   6 &   9 \\ 
  ex1226 & -17.00 & 0.00 &   1 &   1 \\ 
  ex1233 & 201540.00 & 3.00 &  21 &  49 \\ 
  ex1243 & 135552.00 & 2.00 &  18 &  47 \\ 
  ex1244 & 95046.40 & 1.00 &  13 &  17 \\ 
  ex1252 & --- & --- & --- & --- \\ 
  ex1252a & 143555.00 & 3.00 &  23 &  54 \\ 
  ex1263 & 69.60 & 87.00 & 1665 & 1773 \\ 
  ex1263a & 38.60 & 55.00 & 1101 & 1142 \\ 
  ex1264 & 31.60 & 11.00 & 185 & 222 \\ 
  ex1264a & 10.00 & 5.00 &  90 & 108 \\ 
  ex1265 & 22.30 & 17.00 & 231 & 343 \\ 
  ex1265a & 15.10 & 5.00 &  60 &  87 \\ 
  ex1266 & --- & --- & 72715 & 74554 \\ 
  ex1266a & 16.30 & 1.00 &   7 &  13 \\ 
  ex3pb & 103.58 & 2.00 &  19 &  37 \\ 
  ex4 & 659.57 & 4.00 &  46 &  77 \\ 
  fac1 & 172954000.00 & 10.00 &  85 & 185 \\ 
  fac2 & 407585000.00 & 5.00 &  35 &  97 \\ 
  fac3 & 34789500.00 & 3.00 &  23 &  53 \\ 
  feedtray & -13.41 & 0.00 &   1 &   1 \\ 
  feedtray2 & --- & --- & --- & --- \\ 
  fo7 & 25.60 & 87.00 & 1643 & 1691 \\ 
  fo7\_2 & 40.43 & 13.00 & 171 & 236 \\ 
  fo7\_ar2\_1 & 55.38 & 307.00 & 5449 & 5627 \\ 
  fo7\_ar25\_1 & --- & --- & 67319 & 67538 \\ 
  fo7\_ar3\_1 & 34.49 & 13.00 &  97 & 212 \\ 
  fo7\_ar4\_1 & 41.66 & 1477.00 & 25281 & 25479 \\ 
  fo7\_ar5\_1 & 38.09 & 7.00 &  53 & 110 \\ 
  fo8 & 47.40 & 6.00 &  66 &  99 \\ 
  fo8\_ar2\_1 & --- & --- & 63425 & 63800 \\ 
  fo8\_ar25\_1 & --- & --- & 62646 & 62978 \\ 
  fo8\_ar3\_1 & 45.34 & 36.00 & 469 & 590 \\ 
  fo8\_ar4\_1 & 38.66 & 47.00 & 384 & 529 \\ 
  fo8\_ar5\_1 & 51.84 & 352.00 & 5769 & 5963 \\ 
  fo9 & 52.78 & 7.00 &  60 & 109 \\ 
  fo9\_ar2\_1 & --- & --- & 59417 & 59843 \\ 
  fo9\_ar25\_1 & --- & --- & 57500 & 57912 \\ 
  fo9\_ar3\_1 & 49.40 & 45.00 & 446 & 592 \\ 
  fo9\_ar4\_1 & --- & --- & 57027 & 57468 \\ 
  fo9\_ar5\_1 & 51.17 & 11.00 &  72 & 131 \\ 
  fuel & 8566.12 & 2.00 &  16 &  42 \\ 
  fuzzy & --- & --- &   1 & 10716 \\ 
  gasnet & 6999380.00 & 13.00 &  97 & 194 \\ 
  gastrans & --- & --- & 73821 & 73824 \\ 
  gbd & 2.20 & 0.00 &   1 &   1 \\ 
  gear & 0.00 & 1.00 &   3 &   4 \\ 
  gear2 & 0.01 & 0.00 &   4 &   6 \\ 
  gear3 & 0.00 & 0.00 &   3 &   4 \\ 
  gear4 & 120.67 & 4.00 &  70 &  87 \\ 
  ghg\_1veh & 7.78 & 0.00 &   1 &   1 \\ 
  ghg\_2veh & 7.78 & 0.00 &   1 &   1 \\ 
  ghg\_3veh & 7.77 & 0.00 &   4 &   5 \\ 
  gkocis & -1.41 & 0.00 &   7 &   9 \\ 
  hda & -4322.55 & 5.00 &  18 &  39 \\ 
  hmittelman & 16.00 & 2.00 &  22 &  39 \\ 
  johnall & -222.37 & 4.00 &  54 &  57 \\ 
  lop97ic & 4535.18 & 9.00 &  10 &  31 \\ 
  lop97icx & 4590.48 & 3.00 &  13 &  31 \\ 
  m3 & 55.80 & 2.00 &  21 &  32 \\ 
  m6 & 123.98 & 11.00 & 105 & 206 \\ 
  m7 & --- & --- & 65916 & 66203 \\ 
  m7\_ar2\_1 & --- & --- & 64246 & 64522 \\ 
  m7\_ar25\_1 & --- & --- & 63515 & 63812 \\ 
  m7\_ar3\_1 & --- & --- & 67526 & 67807 \\ 
  m7\_ar4\_1 & 450.97 & 122.00 & 1993 & 2166 \\ 
  m7\_ar5\_1 & 511.21 & 58.00 & 857 & 1025 \\ 
  mbtd & 5.58 & 65.00 &  13 &  41 \\ 
  meanvarx & 14.37 & 2.00 &  23 &  26 \\ 
  meanvarxsc & --- & --- & --- & --- \\ 
  minlphix & 345.51 & 3.00 &  53 &  63 \\ 
  netmod\_dol1 & -0.01 & 16.00 &  22 &  40 \\ 
  netmod\_dol2 & -0.49 & 36.00 &  16 &  44 \\ 
  netmod\_kar1 & 0.00 & 2.00 &  17 &  31 \\ 
  netmod\_kar2 & 0.00 & 2.00 &  17 &  31 \\ 
  no7\_ar2\_1 & --- & --- & 53460 & 53715 \\ 
  no7\_ar25\_1 & 175.87 & 157.00 & 2635 & 2871 \\ 
  no7\_ar3\_1 & 149.22 & 13.00 & 142 & 201 \\ 
  no7\_ar4\_1 & 188.94 & 129.00 & 2040 & 2246 \\ 
  no7\_ar5\_1 & 153.84 & 172.00 & 2440 & 2576 \\ 
  nous1 & 1.57 & 1.00 &   3 &   4 \\ 
  nous2 & 0.63 & 0.00 &   3 &   4 \\ 
  nuclear104 & --- & --- & --- & --- \\ 
  nuclear10a & --- & --- & 1744 & 2063 \\ 
  nuclear10b & -1.15 & 1627.00 &  31 & 124 \\ 
  nuclear14 & -1.13 & 3.00 &   4 &   5 \\ 
  nuclear14a & -1.13 & 1.00 &   1 &   1 \\ 
  nuclear14b & -1.09 & 12.00 &  51 &  73 \\ 
  nuclear25 & -1.12 & 8.00 &  22 &  29 \\ 
  nuclear25a & -1.12 & 5.00 &  22 &  29 \\ 
  nuclear25b & -1.09 & 30.00 &  63 & 153 \\ 
  nuclear49 & -1.15 & 29.00 &  13 &  17 \\ 
  nuclear49a & -1.15 & 25.00 &  25 &  33 \\ 
  nuclear49b & -1.13 & 131.00 &  25 &  74 \\ 
  nuclearva & -1.01 & 4.00 &  33 &  45 \\ 
  nuclearvb & -1.02 & 0.00 &   1 &   1 \\ 
  nuclearvc & -0.98 & 8.00 &  49 &  59 \\ 
  nuclearvd & -1.04 & 6.00 &  63 &  75 \\ 
  nuclearve & -1.02 & 1.00 &   7 &   9 \\ 
  nuclearvf & --- & --- & --- & --- \\ 
  nvs01 & 13.10 & 1.00 &   5 &   7 \\ 
  nvs02 & 5.96 & 2.00 &  35 &  38 \\ 
  nvs03 & 16.00 & 0.00 &  11 &  14 \\ 
  nvs04 & --- & --- & --- & --- \\ 
  nvs05 & 5.47 & 0.00 &   3 &   4 \\ 
  nvs06 & 1.86 & 1.00 &   3 &   4 \\ 
  nvs07 & 4.00 & 0.00 &   5 &   6 \\ 
  nvs08 & 23.83 & 1.00 &  10 &  14 \\ 
  nvs09 & -43.13 & 0.00 &   1 &   1 \\ 
  nvs10 & -308.40 & 0.00 &   4 &   7 \\ 
  nvs11 & -416.40 & 3.00 &  69 &  74 \\ 
  nvs12 & -477.00 & 0.00 &   3 &   5 \\ 
  nvs13 & -585.20 & 0.00 &   3 &   5 \\ 
  nvs14 & -40358.20 & 2.00 &  35 &  38 \\ 
  nvs15 & 1.00 & 0.00 &   3 &   4 \\ 
  nvs16 & 14.20 & 5.00 &  55 & 108 \\ 
  nvs17 & -1078.20 & 3.00 &  52 &  57 \\ 
  nvs18 & -778.40 & 1.00 &   3 &   5 \\ 
  nvs19 & -1070.00 & 1.00 &  10 &  17 \\ 
  nvs20 & 230.92 & 1.00 &   7 &  13 \\ 
  nvs21 & -4.27 & 9.00 & 172 & 174 \\ 
  nvs22 & 6.06 & 0.00 &   4 &   6 \\ 
  nvs23 & -1078.40 & 1.00 &   3 &   5 \\ 
  nvs24 & -1001.00 & 0.00 &   7 &  14 \\ 
  o7 & 190.62 & 23.00 & 374 & 418 \\ 
  o7\_2 & 161.38 & 17.00 & 147 & 281 \\ 
  o7\_ar2\_1 & --- & --- & 66427 & 66695 \\ 
  o7\_ar25\_1 & 160.47 & 165.00 & 2936 & 3100 \\ 
  o7\_ar3\_1 & 162.83 & 33.00 & 446 & 562 \\ 
  o7\_ar4\_1 & 182.29 & 69.00 & 971 & 1138 \\ 
  o7\_ar5\_1 & 166.99 & 80.00 & 1274 & 1443 \\ 
  o8\_ar4\_1 & 345.47 & 26.00 & 130 & 256 \\ 
  o9\_ar4\_1 & 341.57 & 52.00 & 497 & 691 \\ 
  oaer & -1.92 & 0.00 &   4 &   5 \\ 
  oil & -0.87 & 1.00 &   3 &   4 \\ 
  oil2 & -0.73 & 0.00 &   3 &   4 \\ 
  ortez & -9532.04 & 1.00 &  13 &  20 \\ 
  parallel & --- & --- & 65803 & 65803 \\ 
  pb302035 & 4052260.00 & 27.00 &  25 &  34 \\ 
  pb302055 & 4087020.00 & 156.00 & 155 & 200 \\ 
  pb302075 & 4624370.00 & 63.00 &  49 &  77 \\ 
  pb302095 & --- & --- & 3127 & 4614 \\ 
  pb351535 & 5474850.00 & 180.00 & 240 & 306 \\ 
  pb351555 & 5256790.00 & 26.00 &  21 &  41 \\ 
  pb351575 & 6457260.00 & 13.00 &  15 &  21 \\ 
  pb351595 & 11847500.00 & 907.00 & 919 & 1524 \\ 
  prob02 & 112235.00 & 1.00 &  10 &  13 \\ 
  prob03 & 11.00 & 1.00 &  18 &  31 \\ 
  prob10 & 3.45 & 0.00 &   3 &   4 \\ 
  procsel & -1.41 & 0.00 &   5 &   7 \\ 
  product & -2075.33 & 16.00 &  56 & 103 \\ 
  product2 & --- & --- & --- & --- \\ 
  qap & 411560.00 & 6.00 &  13 &  28 \\ 
  qapw & 395664.00 & 46.00 & 106 & 345 \\ 
  ravempb & 269590.00 & 1.00 &  10 &  23 \\ 
  risk2bpb & -55.48 & 2.00 &  17 &  21 \\ 
  saa\_2 & 12.75 & 35.00 &  50 &  78 \\ 
  sep1 & -510.08 & 0.00 &   5 &   7 \\ 
  space25 & 919.99 & 283.00 & 3235 & 4234 \\ 
  space25a & 657.73 & 6.00 &  80 & 106 \\ 
  space960 & 7985000.00 & 104.00 &  39 & 111 \\ 
  spectra2 & 14.04 & 3.00 &  25 &  53 \\ 
  spring & 1.35 & 2.00 &  19 &  27 \\ 
  st\_e13 & --- & --- & --- & --- \\ 
  st\_e14 & 5.81 & 0.00 &   6 &  10 \\ 
  st\_e15 & --- & --- & --- & --- \\ 
  st\_e27 & 2.00 & 0.00 &   1 &   1 \\ 
  st\_e29 & -0.88 & 1.00 &  12 &  19 \\ 
  st\_e31 & --- & --- & --- & --- \\ 
  st\_e32 & -0.72 & 14.00 & 243 & 289 \\ 
  st\_e35 & 71468.10 & 1.00 &   3 &   4 \\ 
  st\_e36 & --- & --- & 8503 & 53584 \\ 
  st\_e38 & 7197.73 & 0.00 &   1 &   1 \\ 
  st\_e40 & --- & --- & --- & --- \\ 
  st\_miqp1 & 380.50 & 1.00 &  15 &  28 \\ 
  st\_miqp2 & 2.00 & 1.00 &  12 &  16 \\ 
  st\_miqp3 & --- & --- & --- & --- \\ 
  st\_miqp4 & --- & --- & --- & --- \\ 
  st\_miqp5 & -333.89 & 0.00 &   1 &   1 \\ 
  stockcycle & 260786.00 & 12.00 & 147 & 218 \\ 
  st\_test1 & 0.00 & 1.00 &   6 &  11 \\ 
  st\_test2 & --- & --- & --- & --- \\ 
  st\_test3 & --- & --- & --- & --- \\ 
  st\_test4 & --- & --- & --- & --- \\ 
  st\_test5 & -110.00 & 2.00 &  28 &  46 \\ 
  st\_test6 & 664.00 & 4.00 &  46 &  75 \\ 
  st\_test8 & -29605.00 & 0.00 &   4 &   5 \\ 
  st\_testgr1 & -12.76 & 1.00 &  11 &  15 \\ 
  st\_testgr3 & -20.50 & 1.00 &  19 &  29 \\ 
  st\_testph4 & -80.50 & 0.00 &   3 &   5 \\ 
  super1 & --- & --- & --- & --- \\ 
  super2 & --- & --- & --- & --- \\ 
  super3 & --- & --- & --- & --- \\ 
  super3t & --- & --- & --- & --- \\ 
  synheat & 219858.00 & 2.00 &  18 &  43 \\ 
  synthes1 & 7.09 & 1.00 &   8 &  14 \\ 
  synthes2 & 80.29 & 1.00 &  17 &  34 \\ 
  synthes3 & 82.37 & 2.00 &  14 &  28 \\ 
  tln12 & 315.60 & 186.00 & 2860 & 3350 \\ 
  tln2 & 23.30 & 16.00 & 284 & 313 \\ 
  tln4 & 9.30 & 5.00 &  92 & 103 \\ 
  tln5 & 16.50 & 4.00 &  47 &  65 \\ 
  tln6 & 20.50 & 9.00 & 177 & 209 \\ 
  tln7 & 39.00 & 165.00 & 3173 & 3239 \\ 
  tloss & 24.30 & 3.00 &  41 &  62 \\ 
  tls12 & --- & --- & 39937 & 48574 \\ 
  tls2 & 11.30 & 211.00 & 3385 & 3543 \\ 
  tls4 & 22.00 & 475.00 & 9538 & 9781 \\ 
  tls5 & 15.50 & 81.00 & 1319 & 1590 \\ 
  tls6 & 36.10 & 191.00 & 2418 & 2859 \\ 
  tls7 & 48.80 & 1641.00 & 27458 & 28995 \\ 
  tltr & 54.60 & 1.00 &  23 &  32 \\ 
  uselinear & --- & --- & --- & --- \\ 
  util & 999.84 & 2.00 &  34 &  39 \\ 
  var\_con10 & 452.69 & 1.00 &   5 &   7 \\ 
  var\_con5 & 285.87 & 1.00 &   3 &   4 \\ 
  waste & 1169.08 & 21.00 &  82 & 139 \\ 
  water3 & --- & --- & --- & --- \\ 
  water4 & 1323.97 & 68.00 & 1294 & 1381 \\ 
  waterful2 & --- & --- & --- & --- \\ 
  waters & --- & --- & --- & --- \\ 
  watersbp & --- & --- & --- & --- \\ 
  watersym1 & --- & --- & --- & --- \\ 
  watersym2 & --- & --- & --- & --- \\ 
  waterx & 934.86 & 0.00 &   7 &  12 \\ 
  waterz & 315610.00 & 1544.00 & 13551 & 26704 \\ 
  windfac & 0.25 & 2.00 &  26 &  28 \\ 
  \end{longtable}

